Is a Video worth $n\times n$ Images? A Highly Efficient Approach to Transformer-based Video Question Answering

Conventional Transformer-based Video Question Answering (VideoQA) approaches generally encode frames independently through one or more image encoders followed by interaction between frames and question. However, such schema would incur significant memory use and inevitably slow down the training and inference speed. In this work, we present a highly efficient approach for VideoQA based on existing vision-language pre-trained models where we concatenate video frames to a $n\times n$ matrix and then convert it to one image. By doing so, we reduce the use of the image encoder from $n^{2}$ to $1$ while maintaining the temporal structure of the original video. Experimental results on MSRVTT and TrafficQA show that our proposed approach achieves state-of-the-art performance with nearly $4\times$ faster speed and only 30% memory use. We show that by integrating our approach into VideoQA systems we can achieve comparable, even superior, performance with a significant speed up for training and inference. We believe the proposed approach can facilitate VideoQA-related research by reducing the computational requirements for those who have limited access to budgets and resources. Our code will be made publicly available for research use.

==> Tables/Table-2-Number-of-Frames.tex <==
\begin{table}
\resizebox{\linewidth}{!}{
\begin{tabular}{lccc}
\toprule
Number of Frames & Multi-Frame & Combine-Frame   \\ \midrule

1 & 88.2 & 88.2 \\

2 & 88.2 & 88.2 \\

3 & 88.2 & 88.2 \\

3 & 88.2 & 88.2 \\

4 & 88.2 & 88.2 \\

5 & 88.2 & 88.2 \\

6 & 88.2 & 88.2 \\

\bottomrule

\end{tabular}
}
\caption{Evaluation results on the effect of amount of video frames on MSRVTT-MC.}
\label{table:results_frame_number}
\end{table}
